InternEvo: Efficient Long-sequence Large Language Model Training via Hybrid Parallelism and Redundant Sharding

Large language models (LLMs) with long sequences begin to power more and more fundamentally new applications we use every day. Existing methods for long-sequence LLM training are neither efficient nor compatible with commonly-used training algorithms such as FlashAttention. We design InternEvo to address these issues. InternEvo decouples all of the sharding dimensions into a new hierarchical space, and systematically analyzes the memory and communication cost of LLM training. Then, it generates an effective hybrid parallelism strategy. We design a new selective overlap mechanism to mitigate the communication overhead introduced by the hybrid parallelism. We also implement memory management techniques to reduce GPU memory fragmentation. Evaluation results show that InternEvo generates parallelization strategies that match or outperform existing methods in model FLOPs utilization.

==> sections/discussion.tex <==
\section{Discussion}
lessons, future directions, etc.




% %%%%%%%%%%%%%%%%%%%% Sunpeng





% Constraints:

% GPU number
% \begin{equation*}
% pp \times sp \times dp = N
% \end{equation*}





% GPU Memory
% \begin{equation*}
% \textstyle \frac{4L\Psi}{pp \times tp \times ps} + \frac{6L\Psi}{pp \times tp \times ps  \times oss} + \frac{M_{\{ACT\}}(sp=pp=1)}{pp \times sp} \leq \text{MaxMem}
% \end{equation*}

% %%%%%%%%%%%%%%%%%%%% Sunpeng

==> sections/implementation.tex <==
\section{Implementation 0.5P}
We have implemented a system prototype for \sysname{} with \todo{xxx} lines of code in \todo{C++ and Python}, including xxx LOC for the the \sysname{} Strategy Planner and XXX LOC for the \sysname{} Job Executor. 
The \sysname{} Job Executor is integrated with InternLM~\cite{InternLM}, an open-sourced lightweight training framework for LLMs.

\parabf{\sysname{} tensor parallelism.}
\todo{how to overlap? (buckets and queues for communication operators, the new functions that we implemented, etc.) how to schedule the collective operators?}

\parabf{Memory pool.}
\todo{how to reorganize the memory blocks? Do we use an extra thread or scheduler?}

==> sections/introduction_deprecated.tex <==
\section{Introduction}
Large language models (LLMs) with long sequences have powered many fundamentally new applications we use every day, including generative AI~\cite{ni2023recent}, long-context understanding~\cite{beltagy2020longformer, zhou2021document}. With the recent emerging ChatGPT, long dialogue processing tasks has become more important for chat applications than ever~\cite{touvron2023llama}.
Despite these scenarios for language processing, transformer-based large models also achieve impressive performance in computer vision~\cite{zhang2020span, arnab2021vivit, yuan2021tokens} and AI for science~\cite{bi2023accurate, ai4science}, where inputs with long sequences are critical for tasks such as processing video streams~\cite{ruan2022survey} and protein property prediction~\cite{chandra2023transformer}.

However, training LLMs with long sequences requires massive memory footprints. 
To train LLMs with long sequences while not sacrificing training speed significantly, several efforts have been proposed to alleviate the memory pressure~\cite{korthikanti2023reducing, jacobs2023deepspeed, liu2023ring, li2023lightseq, li2021sequence}. However, these methods suffer from two limitations. 
On one hand, some current methods are not good enough in scaling sequence length and model size~\cite{korthikanti2023reducing, li2021sequence}. The GPU memory and communication bandwidth can be further efficiently utilized to support longer sequence length and larger model size.
On the other hand, existing methods are not efficient enough in training performance. Many methods reduce the required memory through activation recomputation~\cite{chen2016training} or distributing data across devices~\cite{jacobs2023deepspeed, li2023lightseq}, which introduces inevitable computation or communication overhead. For example, DeepSpeed Ulysses~\cite{jacobs2023deepspeed} requires frequent communications between different servers through networking, whose bandwidth is usually low. Furthermore, despite the importance of long sequence training, training with short sequences is essential and nonnegligible.
The communication overhead is even more severe on training with short sequences~\cite{li2023lightseq}.

In this paper, we propose \sysname{}, a new tensor parallelism solution for memory-efficient and communication-efficient LLM training. \sysname{} can train LLMs on large model size and longe sequence length, while achieving high throughputs in both short and long sequence training. 
The key idea partition the sequence and model parameter tensors at the same time and distribute them across devices to fit into device memory. 
This significantly reduces the activation and parameter memory usage. 
Then, to ensure the computations are correct, we gather the scattered model parameters into global ones before the Attention, Linear, and MLP computation. 

Although this parallelism solution reduces the memory requirement of each GPU device for long sequence training, the communication required by \sysname{} brings two challenges. First, \sysname{} introduces extra communication overheads. The overheads slow down the training, especially with shorter sequence length. 
Second, \sysname{} requires a large number of collective communications of small tensors. These communications lead to frequent memory allocations and releases, which further introduce GPU memory fragmentations. Therefore, the GPU memory cannot be fully utilized. 

To address these challenges, we first design a selective computation-communication overlap strategy to hide the communication introduced by \sysname{} sufficiently. By prefetching the data required by the next block or next module, \sysname{} hides the non-blocking communications into computation.
Then, to reduce the scattered memory fragments, \sysname{} builds a memory pool for unified memory management. By managing frequent allocations and releases of small memory pieces, contiguous memory is saved for large memory blocks. This enables training on longer sequence lengths without the memory management techniques such as activation checkpoint and offloading, which slows down training.

In summary, we make the following contributions:
\begin{itemize}
\item We propose \sysname{}, a novel tensor parallelism solution which enables efficient long sequence training on LLMs.
\item We design a selective communication-computation overlap strategy that sustains high training throughput.
\item We introduce a novel memory management method, which builds a memory pool to avoid memory fragmentation.
\item We implement a system prototype and integrate it with InternLM\cite{InternLM}. Evaluation results on \todo{xxx models} show that compared to competitive baselines, \sysname{} trains LLMs with \todo{xxx} speedup at most.
\end{itemize}

